Jet substructure in ATLAS

Measurements are presented of the jet invariant mass and substructure in proton-proton collisions at sqrt{s} = 7 TeV with the ATLAS detector using an integrated luminosity of 37 pb-1. These results exercise the tools for distinguishing the signatures of new boosted massive particles in the hadronic final state. Two "fat" jet algorithms are used, along with the filtering jet grooming technique that was pioneered in ATLAS. New jet substructure observables are compared for the first time to data at the LHC. Finally, a sample of candidate boosted top quark events collected in the 2010 data is analyzed in detail for the jet substructure properties of hadronic "top-jets" in the final state. These measurements demonstrate not only our excellent understanding of QCD in a new energy regime but open the path to using complex jet substructure observables in the search for new physics.

==> sec-shapes.tex <==
Hadronic event shapes are constructed as normalized ratios of combinations of hadronic jets. This definition offers several advantages over the explicit cross-section calculations for inclusive single and multi-jet production. Sensitivity to experimental uncertainties such as the jet energy scale are reduced significantly. Various choices of event shape can also lead to enhanced or suppressed sensitivity to different components of the fundamental physical processes involved, such as the underlying event, the parton shower, or the choice of renormalization and factorization scales. \ytwoth represents the threshold at which the event transitions from a di-jet event into a multi-jet (specifically three-jet) event is defined as $\ytwoth = \dtwoth/\Qsq$, where $\dtwoth = p^2_{t,3}$ and $\Qsq = (p_{t,1}+p_{t,2})^2$. The sphericity, \sph~\cite{Bjorken1970}, transverse sphericity, \sphtranv, and aplanarity, \apla~\cite{Barate19981}, all embody more global information about the full momentum tensor of the event via its eigenvalues $\lambda_1$, $\lambda_2$ and $\lambda_3$: $\sph \equiv \frac{3}{2}(\lambda_2 + \lambda_3)$, $\sphtranv \equiv \frac{2\lambda_2}{\lambda_1 + \lambda_2}$, and $\apla \equiv \frac{3}{2}\lambda_3$. The transverse thrust, $T_{\perp}$ , and its minor component, \thrmin, attempt to define explicitly a thrust axis for the event that maximizes the total transverse momentum  of the event. These quantities are defined as $\thrmaj \equiv 1 - T_{\perp}$ where $T_{\perp} \equiv \max_{\thrvec} \frac{\sum_i |{\vec q}_{\perp i}\cdot {\thrvec}|}{\sum_i q_{\perp i}}$, and  $\thrmin \equiv \frac{\sum_i |{\vec q}_{\perp i}\times {\thrvec}|}{\sum_i q_{\perp i}}$.

Event shape measurements with detector-to-hadron level corrections derived using the \Alpgen generator are shown in Figures~\ref{fig:eventshapes:unfolded1}-\ref{fig:eventshapes:unfolded3}. These corrections account for detector inefficiencies and modeling of the real detector. Systematic uncertainties are assessed for the jet energy scale, pile-up effects, and Monte Carlo variations in the detector-to-hadron level corrections. \Alpgen, \Herwigpp, and \PythiaP all describe the measured event shapes well. All three MC programs have been evaluated for their impact on these corrections and have been shown to yield similar results. Some discrepancies are observed particularly in the tails of steeply falling distributions, such as the aplanarity, or in the transverse thrust. 

The three-jet resolution and aplanarity are both shown in Figure~\ref{fig:eventshapes:unfolded1}. In the case of \ytwoth, where the primary sensitivity is to the parton shower or matrix element description of the momentum of the third jet, \Herwigpp exhibits slightly better agreement with the data. Although \Alpgen provides exact matrix element calculations for up to 6 jets, a slight overestimation of events with low \lny -- or equivalently a low \pTthree to \HT\ ratio -- is observed. This indicates that despite the more precise calculation of the high jet multiplicity states, the impact of tuning the parton shower simulation plays a significant role. The aplanarity on the other hand measures the sum of the transverse momenta out of the event plane defined primarily by the two hardest jets. Although a steeply falling distribution, the deviation of the MC prediction from the data is statistically significant for both \PythiaP and \Herwigpp. The measurements consistently support more highly ``aplanar'' events than predicted by \Herwigpp and fewer than \PythiaP indicates, although the statistical significance of the latter discrepancy is not high. The agreement with \Alpgen is good throughout the range of phase space probed in a statistically significant way. These results suggest that the topological distribution of the event shape is more accurately described by the exact multi-jet prediction provided by the matrix element MC even though \Herwigpp is seen to match the three-jet resolution more accurately.
%%------------------------------    
\begin{figure}%[!ht]
  \centering
%%%% lny23  
  \subfigure[\lny]{
    \includegraphics[width=0.48\columnwidth]{DataMC/unfolded_lny23_Alpgen_v12.pdf}
    \label{fig:eventshapes:unfolded:lny23}}
%%%% aplanarity  
  \subfigure[\apla]{
    \includegraphics[width=0.48\columnwidth]{DataMC/unfolded_aplanarity_Alpgen_v12.pdf}
    \label{fig:eventshapes:unfolded:apl}}
  \caption{Unfolded hadron level measurements of the
           \subref{fig:eventshapes:unfolded:lny23} three-jet resolution, \lny, and
           \subref{fig:eventshapes:unfolded:apl} aplanarity, \apla. 
           The unfolding is performed using the \Alpgen generator with pile-up added.
           }
  \label{fig:eventshapes:unfolded1}
\end{figure}
%%------------------------------ 

The hypothesis that the topological distribution is more well described by \Alpgen is supported by the measurement of the transverse thrust, \thrmaj. Figure~\ref{fig:eventshapes:unfolded:thrustMajor} exhibits the same qualitative discrepancy as observed in the aplanarity: \Herwigpp predicts fewer highly isotropic events (i.e. fewer high \apla or high \thrmaj events) than observed. However, it should be noted that at small but significantly non-zero thrust, \Herwigpp fares much better than \Alpgen and \Pythia where significant ($\mathcal{O}(20\%)$) differences can be seen. In this intermediate thrust range, \Alpgen and \Pythia both predict a thrust distribution shifted towards slightly higher values. Due to this improved agreement at low but non-zero thrust, the average agreement between data and the various MC generators is closest for \Herwigpp. The minor component of the thrust, \thrmin, or the out-of-plane thrust magnitude does not readily suggest as large of a discrepancy as observed in the aplanarity.

%%------------------------------    
\begin{figure}%[!ht]
  \centering
%%%% thrust major  
  \subfigure[\thrmaj]{
    \includegraphics[width=0.48\columnwidth]{DataMC/unfolded_thrustMajor_Alpgen_v12.pdf}
    \label{fig:eventshapes:unfolded:thrustMajor}}
%%%% thrust minor  
  \subfigure[\thrmin]{
    \includegraphics[width=0.48\columnwidth]{DataMC/unfolded_thrustMinor_Alpgen_v12.pdf}
    \label{fig:eventshapes:unfolded:thrustMinor}}
  \caption{Unfolded hadron level measurements of the
           \subref{fig:eventshapes:unfolded:thrustMajor} tranverse thrust, \thrmaj, and
           \subref{fig:eventshapes:unfolded:thrustMinor} minor component of the 
           transverse thrust, \thrmin. 
           The unfolding is performed using the \Alpgen generator with pile-up added.
           }
  \label{fig:eventshapes:unfolded2}
\end{figure}
%%------------------------------ 

Lastly, the sphericity and transverse sphericity shown in Figure~\ref{fig:eventshapes:unfolded3} exhibit very little discernible discrepancy between the MC predictions and the data. The construction of these observables as ratios of eigenvalues of the momentum tensor of the event contributes significantly to this agreement.

%%------------------------------    
\begin{figure}%[!ht]
  \centering
%%%% sphericity  
  \subfigure[\sph]{
    \includegraphics[width=0.48\columnwidth]{DataMC/unfolded_sphericity_Alpgen_v12.pdf}
    \label{fig:eventshapes:unfolded:sph}}
%%%% transverse sphericity  
  \subfigure[\sphtranv]{
    \includegraphics[width=0.48\columnwidth]{DataMC/unfolded_transv_sphericity_Alpgen_v12.pdf}
    \label{fig:eventshapes:unfolded:sphtranv}}
  \caption{Unfolded hadron level measurements of the
           \subref{fig:eventshapes:unfolded:sph} sphericity, \sph, and
           \subref{fig:eventshapes:unfolded:sphtranv} transverse sphericity, \sphtranv.
           The unfolding is performed using the \Alpgen generator with pile-up added.
           }
  \label{fig:eventshapes:unfolded3}
\end{figure}
%%------------------------------ 

